Phantom cascades: The effect of hidden nodes on information diffusion

Research on information diffusion generally assumes complete knowledge of the underlying network. However, in the presence of factors such as increasing privacy awareness, restrictions on application programming interfaces (APIs) and sampling strategies, this assumption rarely holds in the real world which in turn leads to an underestimation of the size of information cascades. In this work we study the effect of hidden network structure on information diffusion processes. We characterise information cascades through activation paths traversing visible and hidden parts of the network. We quantify diffusion estimation error while varying the amount of hidden structure in five empirical and synthetic network datasets and demonstrate the effect of topological properties on this error. Finally, we suggest practical recommendations for practitioners and propose a model to predict the cascade size with minimal information regarding the underlying network.

==> inc/qualitativeAnalysis.tex <==
\begin{figure*}[!htbp]
    \begin{center}







\hspace{-0.5cm}\includegraphics[width=1.02\textwidth]{fig/u_v_h.pdf}
     
    \vspace{-0.5cm}
    \caption{\small Hidden, observed and {\un } cascade fractions as a function of the fraction of hidden nodes $\rho$.}
    \label{fig:3ds}
    \end{center}
    \vspace{-0.7cm}
\end{figure*}

























To understand the interaction between the different cascade types and their effect on the spread residual, we plot the observed, hidden and {\un } cascade sizes as fractions of the total cascade size in Figure~\ref{fig:3ds}.



We note the following observations: i) the hidden cascade grows linearly as a consequence of the uniform sampling, ii) the observed cascade size decreases as $\rho$ increases, steeply in some cases (e.g., Facebook NY) and then plateaus as more nodes are hidden, iii) as $\gamma$ increases, the observed cascade size both grows (because the seeds are drawn from the visible nodes) and exhibits a more linearly decreasing trend as $\rho$ increases. Similarly, the {\un } cascade shrinks significantly for higher seed sizes, resulting in a smaller spread residual.


We now examine the behaviour of the {\un } and observed cascades with respect to the different datasets. As $\rho$
approaches $0.3$ the {\un } cascade grows for all networks. This is expected because as more nodes become hidden, the
probability that a visible node is activated through a path containing a hidden node (i.e., becomes \un) increases. However, as $\rho$ increases even further the size of the {\un } cascade has different behaviour between the datasets. We explain this behaviour as follows:



 
\para{Facebook NY, Astro Physics and 2.5K.} As $\rho$ approaches 0.3, the {\un } cascade size starts to decrease and plateau. This trend is due to the slowing descent of the observed cascade.  Indeed, the observed cascade exhibits a  lower-bound threshold  which is  the number of  nodes directly approached from the seed. 

Recall that Figure~\ref{fig:firstHopDiffusion} showed the fraction of  nodes activated observably and directly from the seeds for the real datasets. Figure~\ref{fig:syncs} depicts this fraction for the synthetic networks, and we show that 2.5K has a similar trend to Astro Physics. Facebook NY, however, exhibits the highest increase in {\un } cascade as $\rho$ increases. This is explained by the long cascade shape presented in Figure~\ref{fig:clustering_by_level}. 







\para{DBLP and TOSHK.} For these networks the {\un } cascade increases very slowly and almost immediately plateaus. This is because the number of  visible nodes that are reached directly from the seeds is larger (Figures~\ref{fig:firstHopDiffusion} and \ref{fig:syncs}), thus contributing to a much higher lower-bound in the observed cascade. % As a result the cascade trees are much wider in breadth and shorter in length reducing the likelihood of a visible node being activated through a hidden path dramatically.

 
\para{Erd\H{o}s-R\'{e}nyi.} Finally, diffusions on the Erd\H{o}s-R\'{e}nyi graph result in extremely shallow cascade trees and are relatively unnaffected by seed size. This is because this random graph lacks any semblance of the social structure shown to influence cascade size and shape. As the diffusion ends much earlier, the {\un } cascade is minimised while the majority fraction of the total cascade remains visible due to counting the seeds as observed cascade.
\para{}

To summarise, we have shown that  {\un } cascades play a crucial role when the cascade trees are long, corresponding to the diffusion process on classes of social networks where the clustering coefficient is low (i.e., such as Facebook NY). Our analysis has shown that for the large seed sizes the effect of the {\un } cascade is minimal and thus the estimation error is lower. Furthermore, when the seed size is relatively small, the {\un } cascade is an important factor to take into account especially for smaller fractions of hidden nodes. In other words, for a higher fraction of hidden nodes the majority of the cascade is, by extension, hidden. This understanding of the interactions between the visible and {\un } cascades enables us to build a correction model that estimates the total cascade size of the oracle with minimal knowledge of the underlying oracle network.




 \begin{figure}[!htbp]
    \begin{center}
 \hspace{-0.5cm}\includegraphics[width=0.5\textwidth]{fig/firstHopDiffusion-syn.pdf}
     
    \vspace{-0.5cm}
    \caption{\small Fraction of nodes that were observably activated at time 0 (seeds) and 1 (directly from the seeds) for the three seed sizes (columns) for the synthetic networks.}
    \label{fig:syncs}
    \end{center}
    \vspace{-0.7cm}
\end{figure}






 









==> inc/results_emprical.tex <==
\section{Results}\label{sec:experimental_result}

In this section we report on the results obtained through empirical evaluation of ICM in partial network.  We first concentrate on the  the overall improvement that is brought by the hidden part of the oracle network  in comparison with the partial network. 
We quantify this improvement by measuring the mean Spread Residual, that is the number of visible nodes that have been activated in oracle network in ratio to those activated in the partial network. Figure~\ref{fig:residuals} illustrates this results for the three real datasets with varying percentage of hidden nodes in the network. 

\begin{figure*}[!ht]
    \begin{center}
    \subfigure[Astro Physics]{\includegraphics[width=0.3\textwidth]{fig/Astro-residual-Exp1.pdf}}
    \subfigure[Facebook NY]{\includegraphics[width=0.3\textwidth]{fig/Facebook-residual-Exp1.pdf}}
     \subfigure[DBLP]{\includegraphics[width=0.3\textwidth]{fig/DBLP-residual-Exp1.pdf}}
    \caption{Mean Spread Residual for diffusion with smallest seed size (0.0001)}
    \label{fig:residuals}
    \end{center}
\end{figure*}


As it can be commonly observed, the spread residual increases exponentially with the increase of hidden part of the network. 
Furthermore, although the trend seems to be the same for all the three networks, the magnitude of the spread residual differs greatly. That is for dense networks such as DBLP and Facebook, the improvement is at most up to 6 (DBLP) and 10 (Facebook)  times than the partial network alone, whereas in case of Astro Physics, such improvement can go up to 40 times. This variation of spread residual amongst different networks is explained by the connectivity of each network. In case of DBLP and Facebook, both networks exhibit high degree connectivity allowing the visible nodes in the partial network have various edges each of which might increasing the chances of activation even without the help of the hidden nodes. In the case of Astro Physics, where the network is not as connected, the mean spread residual as well as standard deviation can span very high reflecting the magnitude by which visible nodes in  the partial network fall short in activation in comparison to the oracle. 




To understand the causation of these results we study the effect of the seed size and hidden nodes on the  hidden, visible and unobserved cascades.  For the  purpose  of this analysis we only considered the discount degree seed selection as random seed selection is not representative of real case. Figure~\ref{fig:astrocascades} presents the behaviours of different cascades  for increasing the  hidden percentage of nodes and for smallest seed size for Astro network graph.


\begin{figure}[h]
\begin{center}
\includegraphics[width=0.5\textwidth]{fig/astro_dd_ts0001_wv1.pdf}
\caption{default}
\label{fig:astrocascades}
\end{center}
\end{figure}

\noteam{observation regarding the 3 cascades goes here}


To study whether the same property holds in different networks (both synthetic and real), we have measured the unobserved cascade fraction while varying seed size and hidden percentage. It is worth noting that due to the space limitation and the high number of figures to report, we have avoided  reporting the results of the hidden and visible cascade as they both can be inferred by  the trend of  unobserved cascade. That is as seen in Figure~\ref{fig:astrocascades}, the hidden cascade grows linearly as  $\rho$ increases,  and the visible cascade mirrors the unobserved cascade trend by first decreasing fast  as $\rho$ increases, and stabilising for higher percentage of hidden nodes. 


\begin{figure*}[!ht]
    \begin{center}
    \subfigure[Astro Physics]{\includegraphics[width=0.2\textwidth]{fig/3dPlaceHolder.pdf}}
    \subfigure[Facebook NY]{\includegraphics[width=0.2\textwidth]{fig/3dPlaceHolder.pdf}}
     \subfigure[DBLP]{\includegraphics[width=0.2\textwidth]{fig/3dPlaceHolder.pdf}}
     \\
         \subfigure[Random]{\includegraphics[width=0.2\textwidth]{fig/3dPlaceHolder.pdf}}
    \subfigure[Toshk]{\includegraphics[width=0.2\textwidth]{fig/3dPlaceHolder.pdf}}
     \subfigure[DK2.5]{\includegraphics[width=0.2\textwidth]{fig/Dk25_ucf_3d_dd.pdf}}
     
    \caption{The effect of seed size and hidden percentage on the unobserved cascade size}
    \label{fig:3ds}
    \end{center}
\end{figure*}




Figure~\ref{fig:3ds} illustrates the impact of target seed size and hidden percentage on unobserved cascade for the six datasets at hand. We discuss these effects in details next.





\para{Seed Size.}  From the Figure~\ref{fig:3ds} we can obsereved that as the seed size increases (The z axis in log scale) the effect of the unobserved cascade decreases. 






\para{Hidden Nodes.} Explain the increase and the drop that is consistently found in the (same 3 cascade size plots as before). Presented as the x axis of the 3d bar chart. 
 Hypothesis: this behavior may be the results on when we hit the hidden nodes in the cascade depth. In particular, we may formulate the following question: {\em Which are the causes of the drop after the 20\%?} Point forward for theoretical understanding. 



\noteam{A paragraph here to emphsize our foundings: a) if you are starting with big seed size, the unobserevd cascade is of a small effect. if you are having too much of the network hidden the unobsereved effect will decrease as most will go to the hidden cascade. also here we should have a paragraph on the global infection probability with i) explaining the effect of increasing this probability, ii) what we expect if the probability was not global but we had weighted cascades.}





\fixme{ - Step 2 (connect to step 1 in previous section) model cascades depth vs breadth using the figures afra provided. Fitting the data!(Alessandra, Donn)

\para{Modeling Cascade Shapes.} depth vs breadth ... Hey Donn, how do we organize the tasks to complete this task? 
}


==> inc/results_emprical2.tex <==
\section{Results}\label{sec:experimental_result}
\noteam{please help in coming up with better section and subsection names for this part. }

\notedm{I think we can make this section work without subheadings}

In this section we report on the results of quantifying the effect of incomplete networks on diffusion process, obtained through empirical evaluation of datasets described in Section \ref{sec:methodology}.  We first motivate the research problem by demonstrating the magnitude of the impact on the diffusion cascade under missing data. We then present a qualitative study of what causes contribute to the observed impact by detail investigation of the diffusion process. 



\subsection{Magnitude of the problem}

For each dataset, we present the degree of error associated with estimating the number of activated nodes in the partial network. To this end, we measure the \emph{spread residual} as described earlier in Section~\ref{sec:methodology}. This metric corresponds to the number of visible nodes which \emph{would have} been activated given the knowledge about the oracle network over the number of nodes that were activated as a result of diffusion in the partial network only.  Intuitively this ratio corresponds to the magnitude of mis-estimation of the number of activated visible nodes when the hidden part of the network is unaccounted for. 

It is worth noting that prior to this paper, \cite{Cebrian:2009:WAY:1641389.1641391} had also attempted to measure this degree of mis-estimation. However, we believe that our approach permits quantifying the error  more accurately than previously done so. This is because our approach allows us  to measure not only what is observed by looking solely at partial network but also  to distinguish between unobserved and hidden cascades (i.e., the type of the nodes that become active as a result of a hidden path). Distinguishing unobserved nodes from those of hidden allows us  to account for  what \emph{would have} happened to the very same visible nodes in the partial network if the knowledge of the oracle network was available. The previous attempt however has only been able to measure the cascade size in the oracle network without  differentiating  between hidden and visible nodes, which indirectly translates to comparing cascades sizes of the partial network with a bigger network. 


\begin{figure*}[!ht]
    \begin{center}
    \subfigure[Astro Physics]{\includegraphics[width=0.3\textwidth]{fig/Astro-residual.pdf}}
    \subfigure[Facebook NY]{\includegraphics[width=0.3\textwidth]{fig/Facebook-residual.pdf}}
     \subfigure[DBLP]{\includegraphics[width=0.3\textwidth]{fig/DBLP-residual.pdf}}
    \caption{Mean Spread Residual for various seed size for networks of different partiality}
    \label{fig:residuals}
    \end{center}
\end{figure*}

 Figure~\ref{fig:residuals} illustrates this results for the three real datasets while the varying percentage of hidden nodes in the network, where spread residual higher than 1 corresponds to the potential that more visible nodes in comparison to those observed from running the diffusion on partial network would have been activated if the hidden part of the network was accounted for.  As it can be commonly observed, the spread residual increases exponentially with the increase of hidden parts of the network. From this figure, we can also observe that as the number of original target seed size increases the mean spread residual decreases and for such cases the spread residual exhibits a linear growth as $\rho$ increases. This is an important observation which can be explained as follows: as the seeds are selected from amongst visible nodes themselves, the higher seed size translates into a higher number of nodes being activated in the partial network thus narrowing the gap with what would have happened in the oracle network. Intuitively, selecting a big enough number of seeds to start with will result in spread residual equal to 1 which means every visible node in the  network has been activated regardless of having the oracle knowledge. 
 
 
 Although one might claim that increasing the number of selected seeds can remove the problem caused by the mis-estimation of the cascade size, we would like to point out that such a strategy is not always possible. As an example, imagine an advertising company which is planning to promote a product for New Yorkers through  Facebook, in this case the strategy of increasing the seed size to a big enough sample to reduce the mis-estimation may not be a possible option as a seed size of 0.01 translates to 10K users whom need to be provoked and be given free samples of the product.  Moreover, from a research perspective, previous literature on information diffusion and seed optimisation has taken 0.0001 as a guideline for the number of the seeds\cite{} 
 
  
 
Furthermore, although the trend seems to be the same for all the three networks, the magnitude of the spread residual differs greatly. That is for dense networks such as DBLP and Facebook, the degree of the error in estimating the cascade size is at most up to 6 (DBLP) and 10 (Facebook)  times, whereas in case of Astro Physics, such degree can go up to 40 times. This variation of spread residual amongst different networks is explained by the connectivity of each network. In case of DBLP and Facebook, both networks exhibit high degree connectivity allowing the visible nodes in the partial network have various edges each of which might increasing the chances of activation even without the help of the hidden nodes. In the case of Astro Physics, where the network is not as connected, the mean spread residual as well as standard deviation can span very high reflecting the magnitude by which visible nodes in  the partial network fall short in activation in comparison to the oracle. 

\noteam{Here we need the justification for the above claim based on connected component and path redundancy}
















\subsection{Qualitative analysis}
We continue our  investigation of  the diffusion cascades in the partial network. Figure~\ref{fig:astrocascades} presents the visible, hidden and unobserved cascade fractions\footnote{We remind the reader that the cascade fractions are normalised to the total cascade size, therefore the sum of three lines adds up to 1.} and interactions amongst them for the Astro Physics network for different seed sizes. Similar results were also obtained for the other five networks but are omitted due to space constraints.


From each subfigure of Figure~\ref{fig:astrocascades} we can observe the following: Intuitively  as the percentage of the hidden nodes in the network increases, the hidden cascade fraction increases linearly, due to hidden nodes being reached earlier in diffusion process and therefore more hidden nodes are activated as the result. This linear effect however is not observed in the visible cascade, but indeed the visible cascade decreases sharply for the smaller $\rho$ values and as more  of the network becomes hidden the visible cascade starts to plateau. This plateau effect can be explained by the decrease in the likelihood of an activation path never ever crossing any hidden nodes.  It is worth noting that for diffusions with higher seed size, the visible cascade both is shifted higher as the seeds are selected from the visible nodes (cascade) and the visible cascade plateau later,as higher number of visible nodes are  activated directly by the seeds themselves.

Let us now focus on unobserved cascade which corresponds to the number of visible nodes that are activated as a result of a hidden node in the diffusion cascade. The impact of increasing $\rho$ on the unobserved cascade is crucial to understand as it quantifies how many visible nodes in the total cascade would have gone unobserved by not knowing the complete network structure.  As Figure~\ref{fig:astrocascades} illustrates the unobserved cascade grows for smaller $\rho$ values, reflecting that as more nodes are hidden in the network more visible nodes become activated through a hidden path. However, this trend reverses for $\rho$ values higher than 0.25; that is when one (or more) nodes out of four  in the oracle network is hidden, the probability of an activated node to also be a hidden node increases resulting in an increase in the hidden cascade than activation of visible nodes (be it through visible or hidden path). This phenomena can be seen clearly by comparing the interactions between three lines. When the $\rho$ ratio increases  as high as one in every two nodes ($\rho=0.5$) in the oracle to be hidden, for the smallest seed size the unobserved and hidden cascade become almost equal each reaching 50\% of the activated nodes. Whilst the visible cascade becomes very low (1\%) and stays limited to those visible nodes which have become activated as direct diffusion from the seeds themselves. 
It is worth noting that the unobserved cascade shrinks significantly for higher seed sizes. That is while hidden cascade follows the same trend for all seed sizes and visible cascade gains more importance, the effect of the unobserved cascade reduces significantly. 





\begin{figure}[h]
\begin{center}
\includegraphics[width=0.5\textwidth]{fig/astro_dd_wv1.pdf}
\caption{Diffusion Cascades of Astro Physics for three different seed sizes}
\label{fig:astrocascades}
\end{center}
\end{figure}


To study whether the same property holds in different networks (both synthetic and real), we have measured the unobserved cascade fraction while varying seed size and hidden percentage. It is worth noting that due to the space limitation and the high number of figures to report, we have avoided  reporting the results of the hidden and visible cascade as Figure~\ref{fig:astrocascades} provided a clear indication of how the other two cascades of visible and hidden vary according to the behaviour of the unobserved cascade.  Figure~\ref{fig:3ds} illustrates these results for the six networks. 




\begin{figure*}[!ht]
    \begin{center}
    \subfigure[Astro Physics]{\includegraphics[width=0.2\textwidth]{fig/astro_u_v_h.pdf}}
    \subfigure[Facebook NY]{\includegraphics[width=0.2\textwidth]{fig/facebook_u_v_h.pdf}}
     \subfigure[DBLP]{\includegraphics[width=0.2\textwidth]{fig/dblp_u_v_h.pdf}}
     \\
         \subfigure[Random]{\includegraphics[width=0.2\textwidth]{fig/erdos_u_v_h.pdf}}
    \subfigure[Toshk]{\includegraphics[width=0.2\textwidth]{fig/toshk_u_v_h.pdf}}
     \subfigure[DK2.5]{\includegraphics[width=0.2\textwidth]{fig/DK_u_v_h.pdf}}
     
    \caption{The effect of seed size and hidden percentage on the unobserved cascade size}
    \label{fig:3ds}
    \end{center}
\end{figure*}





\noteam{A paragraph here to emphsize our foundings: a) if you are starting with big seed size, the unobserevd cascade is of a small effect. if you are having too much of the network hidden the unobsereved effect will decrease as most will go to the hidden cascade. also here we should have a paragraph on the global infection probability with i) explaining the effect of increasing this probability, ii) what we expect if the probability was not global but we had weighted cascades.}







